On Insecure Uses of BGN for Privacy Preserving Data Aggregation Protocols

The notion of aggregator oblivious (AO) security for privacy preserving data aggregation was formalized with a specific construction of AO-secure blinding technique over a cyclic group by Shi et al. Some of proposals of data aggregation protocols use the blinding technique of Shi et al. for BGN cryptosystem, an additive homomorphic encryption. Previously, there have been some security analysis on some of BGN based data aggregation protocols in the context of integrity or authenticity of data. Even with such security analysis, the BGN cryptosystem has been a popular building block of privacy preserving data aggregation protocol. In this paper, we study the privacy issues in the blinding technique of Shi et al. used for BGN cryptosystem. We show that the blinding techniques for the BGN cryptosystem used in several protocols are not privacy preserving against the recipient, the decryptor. Our analysis is based on the fact that the BGN cryptosystem uses a pairing e:GxG-->G_T and the existence of the pairing makes the DDH problem on G easy to solve. We also suggest how to prevent such privacy leakage in the blinding technique of Shi et al. used for BGN cryptosystem.

==> refer.tex <==

\begin{thebibliography}{1}
\providecommand{\url}[1]{\texttt{#1}}
\providecommand{\urlprefix}{URL }
\expandafter\ifx\csname urlstyle\endcsname\relax
  \providecommand{\doi}[1]{doi:\discretionary{}{}{}#1}\else
  \providecommand{\doi}{doi:\discretionary{}{}{}\begingroup
  \urlstyle{rm}\Url}\fi
\providecommand{\eprint}[2][]{\url{#2}}


\bibitem{BGN05}
 Boneh D,  Goh E, and Nissim K.
\newblock Evaluating 2-DNF formulas on ciphertexts.
\newblock TCC 2005.
\newblock LNCS 3378, 2005. pp.~325--342.
doi:10.1007/978-3-540-30576-7\_18.

\bibitem{BL16}
 Bao H, and Lu R.
 Comment on ``Privacy-Enhanced Data Aggregation Scheme Against Internal Attackers in Smart Grid".
 IEEE Transactions on industrial informatics, 2016. 12(1):1–5. doi:10.1109/TII.2015.2500882.

\bibitem{FHL14}
Fan C-I,  Huang S-Y, and Lai Y-L.
\newblock Privacy-Enhanced Data Aggregation Scheme Against Internal Attackers in Smart Grid.
\newblock IEEE Transactions on industrial informatics,
\newblock  2003. 10(1):666--675.


\bibitem{HKZVY17}
 He D, Kumar N,  Zeadally S,  Vinel A, and  Yang L.
\newblock Efficient and Privacy Preserving Data Aggregation Scheme for Smart Grid Against Internal Adversaries.
\newblock IEEE Transactions on smart grid,
\newblock 2017.  8(5):2411--2417.

\bibitem{LLWKR19}
 Li X,  Liu S,  Wu F,  Kumari S, and  Rodrigues J.
\newblock Privacy Preserving Data Aggregation Scheme for Mobile Edge Computing Assisted IoT Applications.
\newblock IEEE Internet of Things Journal,
\newblock 2019.  6(3):4755--4763.


\bibitem{SCRCS11}
 Shi E, Chan T-H, Chan H, Rieffel E, Chow R, and  Song D.
\newblock Privacy-Preserving Aggregation of Time-Series Data.
\newblock NDSS 2011. pp.~483--501.

\bibitem{W17}
 Wang Z.
\newblock An Identity-based data aggregation protocol for the smart grid.
\newblock IEEE Transactions on industrial informatics,
\newblock 2017.  13(5):2428--2435. doi:10.1109/TII.2017.2705218.

\bibitem{WXX18}
 Wang Z,  Xie H, and  Xu Y.
\newblock Security Analysis of an Identity-Based Data Aggregation Protocol for the Smart Grid.
\newblock ISDDC 2018.
\newblock LNCS 11317, 2018. pp.~63--73.  doi:10.1007/978-3-030-03712-3\_6.


\bibitem{ZLC22}
 Zeng Z,  Liu Y, and Chang L.
\newblock A Robust and Optional Privacy Data Aggregation Scheme for Fog-Enhanced IoT Network.
\newblock IEEE Systems Journal, 2022. pp.~1--11. doi:10.1109/JSYST.2022.3177418.

\end{thebibliography}
